Poster: Improving Bug Localization with Report Quality Dynamics and Query Reformulation

Recent findings from a user study suggest that IR-based bug localization techniques do not perform well if the bug report lacks rich structured information such as relevant program entity names. On the contrary, excessive structured information such as stack traces in the bug report might always not be helpful for the automated bug localization. In this paper, we conduct a large empirical study using 5,500 bug reports from eight subject systems and replicating three existing studies from the literature. Our findings (1) empirically demonstrate how quality dynamics of bug reports affect the performances of IR-based bug localization, and (2) suggest potential ways (e.g., query reformulations) to overcome such limitations.

==> README <==
This is the README for the mweights package, version 2016-12-09.

Many font families available for use with LaTeX have multiple
weights, especially when originally aimed at use on the web. For
example, Linux Libertine has both bold and semibold; Cabin, a
sans-serif family, has four weights (regular, medium, semibold,
bold); SourceCodePro, a monospaced family, has seven weights.

Traditionally the type1-oriented support packages for such fonts
re-define the standard \mddefault or \bfdefault macros. But this can
create difficulties if the weight desired for one font family isn't
available for another font family, or if it differs from the weight
desired for another font family. For example, there is no medium
weight font for Linux Libertine so that setting \mddefault to mb for
use with Cabin will be problematic for Libertine. And \bfdefault
cannot be both sb for use with Cabin and b for use with Libertine,
or vice versa.

This package provides a solution to these difficulties. The basic
idea (due to Michael Sharpe) is that font packages should *not*
re-define \mddefault or \bfdefault; instead they should define as
many of the following macros as is appropriate:

\mdseries@rm
\mdseries@sf
\mdseries@tt

\bfseries@rm
\bfseries@sf
\bfseries@tt

For example, 

\def\mdseries@sf{mb}
\def\bfseries@sf{b}

would be appropriate definitions for using a sans font such as Cabin 
with medium and bold, and

\def\bfseries@rm{sb}

would be appropriate for using a Roman font such as Libertine
with semibold. These macros should always be fully expanded; if
necessary, \edef should be used.

The package re-defines standard selection commands for series
(\mdseries and \bfseries) and family (\rmfamily, \sffamily,
\ttfamily) to use the macros. It should be a RequiredPackage (for
type1 font use only) in any such font package.

The package is licensed under the terms of the LaTeX Project Public
License. The maintainer is Bob Tennent (rdt at cs.queensu.ca).  

